Superclustering with the Atacama Cosmology Telescope and Dark Energy Survey: I. Evidence for thermal energy anisotropy using oriented stacking

The cosmic web contains filamentary structure on a wide range of scales. On the largest scales, superclustering aligns multiple galaxy clusters along inter-cluster bridges, visible through their thermal Sunyaev-Zel'dovich signal in the Cosmic Microwave Background. We demonstrate a new, flexible method to analyze the hot gas signal from multi-scale extended structures. We use a Compton-$y$ map from the Atacama Cosmology Telescope (ACT) stacked on redMaPPer cluster positions from the optical Dark Energy Survey (DES). Cutout images from the $y$ map are oriented with large-scale structure information from DES galaxy data such that the superclustering signal is aligned before being overlaid. We find evidence for an extended quadrupole moment of the stacked $y$ signal at the 3.5$\sigma$ level, demonstrating that the large-scale thermal energy surrounding galaxy clusters is anisotropically distributed. We compare our ACT$\times$DES results with the Buzzard simulations, finding broad agreement. Using simulations, we highlight the promise of this novel technique for constraining the evolution of anisotropic, non-Gaussian structure using future combinations of microwave and optical surveys.

==> affiliations.tex <==
\noindent$^1$David A. Dunlap Department of Astronomy \& Astrophysics, University of Toronto, 50 St. George St., Toronto, ON M5S 3H4, Canada\\
$^2$Canadian Institute for Theoretical Astrophysics, University of Toronto, 60 St. George St., Toronto, ON M5S 3H4, Canada\\
$^3$Dunlap Institute of Astronomy \& Astrophysics, 50 St. George St., Toronto, ON M5S 3H4, Canada\\
$^4$School of Earth and Space Exploration, Arizona State University, Tempe, AZ 85287, USA\\
$^5$Perimeter Institute for Theoretical Physics, 31 Caroline Street N, Waterloo ON N2L 2Y5 Canada\\
$^6$Institute for Astronomy, University of Hawai'i, 2680 Woodlawn Drive, Honolulu, HI 96822, USA\\
$^7$Lawrence Berkeley National Laboratory, 1 Cyclotron Road, Berkeley, CA 94720, USA\\
$^8$Department of Physics and Astronomy, University of Pennsylvania, Philadelphia, PA 19104, USA\\
$^9$Kavli Institute for Particle Astrophysics \& Cosmology, P. O. Box 2450, Stanford University, Stanford, CA 94305, USA\\
$^{10}$Berkeley Center for Cosmological Physics, 341 Campbell Hall, University of California, Berkeley, CA 94720, USA\\
$^{11}$Department of Physics, Stanford University, 382 Via Pueblo Mall, Stanford, CA 94305, USA\\
$^{12}$Cerro Tololo Inter-American Observatory, NSF's National Optical-Infrared Astronomy Research Laboratory, Casilla 603, La Serena, Chile\\
$^{13}$Department of Astronomy and Astrophysics, University of Chicago, 5640 S. Ellis Ave., Chicago, IL 60637, USA\\
$^{14}$Kavli Institute for Cosmological Physics, University of Chicago, Chicago, IL 60637, USA\\
$^{15}$Laborat\'orio Interinstitucional de e-Astronomia - LIneA, Rua Gal. Jos\'e Cristino 77, Rio de Janeiro, RJ - 20921-400, Brazil\\
$^{16}$Fermi National Accelerator Laboratory, P. O. Box 500, Batavia, IL 60510, USA\\
$^{17}$Instituto de F\'{i}sica Te\'orica, Universidade Estadual Paulista, S\~ao Paulo, Brazil\\
$^{18}$Department of Astronomy, Cornell University, Ithaca, NY 14853, USA\\
$^{19}$CNRS, UMR 7095, Institut d'Astrophysique de Paris, F-75014, Paris, France\\
$^{20}$Sorbonne Universit\'es, UPMC Univ Paris 06, UMR 7095, Institut d'Astrophysique de Paris, F-75014, Paris, France\\
$^{21}$Department of Physics \& Astronomy, University College London, Gower Street, London, WC1E 6BT, UK\\
$^{22}$School of Physics and Astronomy, Cardiff University, The Parade, Cardiff, CF24 3AA, UK\\
$^{23}$Instituto de Astrofisica de Canarias, E-38205 La Laguna, Tenerife, Spain\\
$^{24}$Universidad de La Laguna, Dpto. Astrofísica, E-38206 La Laguna, Tenerife, Spain\\
$^{25}$Center for Astrophysical Surveys, National Center for Supercomputing Applications, 1205 West Clark St., Urbana, IL 61801, USA\\
$^{26}$Department of Astronomy, University of Illinois at Urbana-Champaign, 1002 W. Green Street, Urbana, IL 61801, USA\\
$^{27}$Institut de F\'{\i}sica d'Altes Energies (IFAE), The Barcelona Institute of Science and Technology, Campus UAB, 08193 Bellaterra (Barcelona) Spain\\
$^{28}$Physics Department, 2320 Chamberlin Hall, University of Wisconsin-Madison, 1150 University Avenue Madison, WI  53706-1390\\
$^{29}$Center for Cosmology and Astro-Particle Physics, The Ohio State University, Columbus, OH 43210, USA\\
$^{30}$Astronomy Unit, Department of Physics, University of Trieste, via Tiepolo 11, I-34131 Trieste, Italy\\
$^{31}$INAF-Osservatorio Astronomico di Trieste, via G. B. Tiepolo 11, I-34143 Trieste, Italy\\
$^{32}$Institute for Fundamental Physics of the Universe, Via Beirut 2, 34014 Trieste, Italy\\
$^{33}$Institut d'Estudis Espacials de Catalunya (IEEC), 08034 Barcelona, Spain\\
$^{34}$Institute of Space Sciences (ICE, CSIC),  Campus UAB, Carrer de Can Magrans, s/n,  08193 Barcelona, Spain\\
$^{35}$Observat\'orio Nacional, Rua Gal. Jos\'e Cristino 77, Rio de Janeiro, RJ - 20921-400, Brazil\\
$^{36}$Department of Physics, University of Michigan, Ann Arbor, MI 48109, USA\\
$^{37}$Centro de Investigaciones Energ\'eticas, Medioambientales y Tecnol\'ogicas (CIEMAT), Madrid, Spain\\
$^{38}$Department of Physics, IIT Hyderabad, Kandi, Telangana 502285, India\\
$^{39}$Faculty of Physics, Ludwig-Maximilians-Universit\"at, Scheinerstr. 1, 81679 Munich, Germany\\
$^{40}$Joseph Henry Laboratories of Physics, Jadwin Hall, Princeton University, Princeton, NJ, USA 08544\\
$^{41}$Department of Astrophysical Sciences, Princeton University, Peyton Hall, Princeton, NJ 08544, USA\\
$^{42}$Santa Cruz Institute for Particle Physics, Santa Cruz, CA 95064, USA\\
$^{43}$Department of Astronomy, University of Michigan, Ann Arbor, MI 48109, USA\\
$^{44}$Department of Physics, Cornell University, Ithaca, NY 14850, USA\\
$^{45}$Instituto de Fisica Teorica UAM/CSIC, Universidad Autonoma de Madrid, 28049 Madrid, Spain\\
$^{46}$Institute of Astronomy, University of Cambridge, Madingley Road, Cambridge CB3 0HA, UK\\
$^{47}$Kavli Institute for Cosmology, University of Cambridge, Madingley Road, Cambridge CB3 0HA, UK\\
$^{48}$Department of Physics, Columbia University, New York, NY, USA 10027\\
$^{49}$Center for Computational Astrophysics, Flatiron Institute, New York, NY, USA 10010\\
$^{50}$Astrophysics Research Centre, University of KwaZulu-Natal, Westville Campus, Durban 4041, South Africa\\
$^{51}$School of Mathematics, Statistics \& Computer Science, University of KwaZulu-Natal, Westville Campus, Durban 4041, South Africa\\
$^{52}$School of Mathematics and Physics, University of Queensland,  Brisbane, QLD 4072, Australia\\
$^{53}$Department of Physics, The Ohio State University, Columbus, OH 43210, USA\\
$^{54}$School of Physics and Astronomy, Sun Yat-sen University, 2 Daxue Road, Tangjia, Zhuhai, 519082, China\\
$^{55}$Department of Physics and Astronomy, Rutgers, the State University of New Jersey, 136 Frelinghuysen Road, Piscataway, NJ 08854-8019, USA\\
$^{56}$Center for Astrophysics $\vert$ Harvard \& Smithsonian, 60 Garden Street, Cambridge, MA 02138, USA\\
$^{57}$Australian Astronomical Optics, Macquarie University, North Ryde, NSW 2113, Australia\\
$^{58}$Lowell Observatory, 1400 Mars Hill Rd, Flagstaff, AZ 86001, USA\\
$^{59}$Departamento de F\'isica Matem\'atica, Instituto de F\'isica, Universidade de S\~ao Paulo, CP 66318, S\~ao Paulo, SP, 05314-970, Brazil\\
$^{60}$George P. and Cynthia Woods Mitchell Institute for Fundamental Physics and Astronomy, and Department of Physics and Astronomy, Texas A\&M University, College Station, TX 77843,  USA\\
$^{61}$Department of Physics, University of Chicago, Chicago, IL 60637, USA\\
$^{62}$Enrico Fermi Institute, University of Chicago, Chicago, IL 60637, USA\\
$^{63}$Instituci\'o Catalana de Recerca i Estudis Avan\c{c}ats, E-08010 Barcelona, Spain\\
$^{64}$Max Planck Institute for Extraterrestrial Physics, Giessenbachstrasse, 85748 Garching, Germany\\
$^{65}$Department of Physics, University of Milano-Bicocca, Piazza della Scienza 3, 20126 Milano (MI), Italy\\
$^{66}$Department of Physics and Astronomy, Pevensey Building, University of Sussex, Brighton, BN1 9QH, UK\\
$^{67}$Department of Physics, University of Arizona, Tucson, AZ 85721, USA\\
$^{68}$Department of Physics, California Institute of Technology, Pasadena, CA 91125, USA\\
$^{69}$Brookhaven National Laboratory, Bldg 510, Upton, NY 11973, USA\\
$^{70}$Instituto de F\'isica, Pontificia Universidad Cat\'olica de Valpara\'iso, Casilla 4059, Valpara\'iso, Chile\\
$^{71}$School of Physics and Astronomy, University of Southampton,  Southampton, SO17 1BJ, UK\\
$^{72}$Computer Science and Mathematics Division, Oak Ridge National Laboratory, Oak Ridge, TN 37831\\
$^{73}$Institute of Cosmology and Gravitation, University of Portsmouth, Portsmouth, PO1 3FX, UK\\
$^{74}$SLAC National Accelerator Laboratory, Menlo Park, CA 94025, USA\\
$^{75}$Universit\"ats-Sternwarte, Fakult\"at f\"ur Physik, Ludwig-Maximilians Universit\"at M\"unchen, Scheinerstr. 1, 81679 M\"unchen, Germany\\
$^{76}$NASA Goddard Space Flight Center, Greenbelt, MD 20771, USA\\
$^{77}$MIT Kavli Institute, Massachusetts Institute of Technology, Cambridge, MA, 02139 USA

==> authors_numbered.tex <==
\correspondingauthor{Martine Lokken}
\email{m.lokken@mail.utoronto.ca}

% main contributors
\author[0000-0001-5917-955X]{M.~Lokken$^{1,2,3}$}
\author[0000-0002-0965-7864]{R.~Hlo\v zek$^{1,3}$}
\author[0000-0002-3495-158X]{A.~van~Engelen$^4$}
\author[0000-0001-6740-5350]{M.~Madhavacheril$^5$}
% data contributors
\author{E.~Baxter$^6$}
\author[0000-0002-0728-0960]{J.~DeRose$^7$}
\author{C.~Doux$^8$}
\author{S.~Pandey$^8$}
\author[0000-0001-9376-3135]{E.~S.~Rykoff$^9$}
\author{G.~Stein$^{10,7}$}
\author[0000-0001-7836-2261]{C.~To$^{11}$}
% alphabetical list of opt-ins, other contributors, and main contributors who were moved out of the top-tier list as per ACT policy
\author{T.~M.~C.~Abbott$^{12}$}
\author[0000-0002-0298-4432]{S.~Adhikari$^{13,14}$}
\author{M.~Aguena$^{15}$}
\author[0000-0002-7069-7857]{S.~Allam$^{16}$}
\author{F.~Andrade-Oliveira$^{17,15}$}
\author[0000-0002-0609-3987]{J.~Annis$^{16}$}
\author[0000-0001-5846-0411]{N.~Battaglia$^{18}$}
\author{G.~M.~Bernstein$^8$}
\author{E.~Bertin$^{19,20}$}
\author[0000-0003-2358-9949]{J.~R.~Bond$^2$}
\author[0000-0002-8458-5047]{D.~Brooks$^{21}$}
\author{E.~Calabrese$^{22}$}
\author[0000-0003-3044-5150]{A.~Carnero~Rosell$^{23,15,24}$}
\author[0000-0002-4802-3194]{M.~Carrasco~Kind$^{25,26}$}
\author[0000-0002-3130-0204]{J.~Carretero$^{27}$}
\author{R.~Cawthon$^{28}$}
\author[0000-0002-5636-233X]{A.~Choi$^{29}$}
\author{M.~Costanzi$^{30,31,32}$}
\author[0000-0002-9745-6228]{M.~Crocce$^{33,34}$}
\author{L.~N.~da Costa$^{15,35}$}
\author{M.~E.~da Silva Pereira$^{36}$}
\author[0000-0001-8318-6813]{J.~De~Vicente$^{37}$}
\author[0000-0002-0466-3288]{S.~Desai$^{38}$}
\author[0000-0002-8134-9591]{J.~P.~Dietrich$^{39}$}
\author{P.~Doel$^{21}$}
\author{J.~Dunkley$^{40,41}$}
\author{S.~Everett$^{42}$}
\author[0000-0002-4876-956X]{A.~E.~Evrard$^{43,36}$}
\author[0000-0003-4992-7854]{S.~Ferraro$^{7,10}$}
\author[0000-0002-2367-5049]{B.~Flaugher$^{16}$}
\author{P.~Fosalba$^{33,34}$}
\author[0000-0003-4079-3263]{J.~Frieman$^{16,14}$}
\author[0000-0001-9731-3617]{P.~A.~Gallardo$^{44}$}
\author[0000-0002-9370-8360]{J.~Garc\'ia-Bellido$^{45}$}
\author[0000-0001-9632-0815]{E.~Gaztanaga$^{33,34}$}
\author[0000-0001-6942-2736]{D.~W.~Gerdes$^{43,36}$}
\author[0000-0002-9865-0436]{T.~Giannantonio$^{46,47}$}
\author[0000-0003-3270-7644]{D.~Gruen$^{39}$}
\author{R.~A.~Gruendl$^{25,26}$}
\author[0000-0003-3023-8362]{J.~Gschwend$^{15,35}$}
\author[0000-0003-0825-0517]{G.~Gutierrez$^{16}$}
\author[0000-0002-9539-0835]{J.~C.~Hill$^{48,49}$}
\author{M.~Hilton$^{50,51}$}
\author[0000-0003-1690-6678]{A.~D.~Hincks$^1$}
\author{S.~R.~Hinton$^{52}$}
\author{D.~L.~Hollowood$^{42}$}
\author[0000-0002-6550-2023]{K.~Honscheid$^{29,53}$}
\author[0000-0002-2571-1357]{B.~Hoyle$^{39}$}
\author{Z.~Huang$^{54}$}
\author[0000-0002-8816-6800]{J.~P.~Hughes$^{55}$}
\author[0000-0001-6558-0112]{D.~Huterer$^{36}$}
\author{B.~Jain$^8$}
\author[0000-0001-5160-4486]{D.~J.~James$^{56}$}
\author{T.~Jeltema$^{42}$}
\author[0000-0003-0120-0808]{K.~Kuehn$^{57,58}$}
\author{M.~Lima$^{59,15}$}
\author[0000-0001-9856-9307]{M.~A.~G.~Maia$^{15,35}$}
\author[0000-0003-0710-9474]{J.~L.~Marshall$^{60}$}
\author{J.~McMahon$^{13,14,61,62}$}
\author[0000-0002-8873-5065]{P.~Melchior$^{41}$}
\author[0000-0002-1372-2534]{F.~Menanteau$^{25,26}$}
\author[0000-0002-6610-4836]{R.~Miquel$^{63,27}$}
\author{J.~J.~Mohr$^{39,64}$}
\author[0000-0001-6606-7142]{K.~Moodley$^{50,51}$}
\author{R.~Morgan$^{28}$}
\author[0000-0002-8307-5088]{F.~Nati$^{65}$}
\author{L.~Page$^{40}$}
\author[0000-0003-2120-1154]{R.~L.~C.~Ogando$^{15,35}$}
\author[0000-0002-6011-0530]{A.~Palmese$^{16,14}$}
\author{F.~Paz-Chinch\'{o}n$^{25,46}$}
\author[0000-0002-2598-0514]{A.~A.~Plazas~Malag\'on$^{41}$}
\author[0000-0001-9186-6042]{A.~Pieres$^{15,35}$}
\author[0000-0002-9328-879X]{A.~K.~Romer$^{66}$}
\author[0000-0002-1666-6275]{E.~Rozo$^{67}$}
\author[0000-0002-9646-8198]{E.~Sanchez$^{37}$}
\author{V.~Scarpine$^{16}$}
\author{A.~Schillaci$^{68}$}
\author[0000-0001-9504-2059]{M.~Schubnell$^{36}$}
\author{S.~Serrano$^{33,34}$}
\author[0000-0002-1831-1953]{I.~Sevilla-Noarbe$^{37}$}
\author{E.~Sheldon$^{69}$}
\author{T.~Shin${^8}$}
\author[0000-0002-8149-1352]{C.~Sif\'on$^{70}$}
\author[0000-0002-3321-1432]{M.~Smith$^{71}$}
\author[0000-0001-6082-8529]{M.~Soares-Santos$^{36}$}
\author[0000-0002-7047-9358]{E.~Suchyta$^{72}$}
\author{M.~E.~C.~Swanson$^{25}$}
\author[0000-0003-1704-0781]{G.~Tarle$^{36}$}
\author{D.~Thomas$^{73,9,74}$}
\author[0000-0001-7211-5729]{D.~L.~Tucker$^{16}$}
\author{T.~N.~Varga$^{64,75}$}
\author[0000-0002-8282-2010]{J.~Weller$^{64,75}$}
\author[0000-0003-2229-011X]{R.~H.~Wechsler$^{11,9,74}$}
\author{R.D.~Wilkinson$^{66}$}
\author[0000-0002-7567-4451]{E.~J.~Wollack$^{76}$}
\author[0000-0001-5112-2567]{Z.~Xu$^{8,77}$}
\collaboration{108}{(Affiliations can be found after the references)}
